Over-parameterized Student Model via Tensor Decomposition Boosted Knowledge Distillation

Increased training parameters have enabled large pre-trained models to excel in various downstream tasks. Nevertheless, the extensive computational requirements associated with these models hinder their widespread adoption within the community. We focus on Knowledge Distillation (KD), where a compact student model is trained to mimic a larger teacher model, facilitating the transfer of knowledge of large models. In contrast to much of the previous work, we scale up the parameters of the student model during training, to benefit from overparameterization without increasing the inference latency. In particular, we propose a tensor decomposition strategy that effectively over-parameterizes the relatively small student model through an efficient and nearly lossless decomposition of its parameter matrices into higher-dimensional tensors. To ensure efficiency, we further introduce a tensor constraint loss to align the high-dimensional tensors between the student and teacher models. Comprehensive experiments validate the significant performance enhancement by our approach in various KD tasks, covering computer vision and natural language processing areas. Our code is available at https://github.com/intell-sci-comput/OPDF.

==> section/table/ablation_table.tex <==
\begin{table*}[t]
\scriptsize
    \centering
        \resizebox{\columnwidth}{!}{
            \begin{tabular}{l|cccccccc|c}
                \hline
                Datasets & \thead{\scriptsize RTE \\ \scriptsize Acc.} &  \thead{\scriptsize MRPC \\ \scriptsize F1/Acc.} &  \thead{\scriptsize STS-B \\ \scriptsize Corr.} &  \thead{\scriptsize CoLA \\ \scriptsize Mcc.} &  \thead{\scriptsize SST-2 \\ \scriptsize F1/Acc.} &  \thead{\scriptsize QNLI \\ \scriptsize Acc.} & \thead{\scriptsize QQP \\ \scriptsize F1/Acc.} &  \thead{\scriptsize MNLI \\ \scriptsize Acc.} & Avg. \\
                \hline
                \rowcolor{gray!10}
                \multicolumn{10}{c}{\textbf{BERT-of-Theseus}} \\
                \hline
                +SVD &  65.5 & 85.4/80.0 & 86.5 & 40.1 & 90.6 & --- & ---/--- & --- & ---\\
                +MPO &  66.1 & 85.6/80.1 & 86.3 & 41.9 & 90.8 & --- & ---/--- & --- & ---\\
                +OPDF  & \textbf{66.2} & \textbf{85.9/80.5} & \textbf{88.6} & \textbf{45.2} & \textbf{ 91.3} & \textbf{89.0} & \textbf{86.8/90.2} & 81.4 & \textbf{80.0} \\
                \hline
                \rowcolor{gray!10}
                \multicolumn{10}{c}{\textbf{LGTM}} \\
                \hline
                +SVD &  64.7 & 86.8/81.9 & 83.1 & 34.4 & 90.1 & 87.9 & 83.5/87.4 & 79.3 & ---\\
                +MPO &  66.2 & 87.4/81.9 & 83.2 & 36.3 & 90.8 & --- & 85.6/89.2 & 79.4 & ---\\
                +OPDF & \textbf{65.5} & \textbf{87.5/82.4} & \textbf{83.3} & \textbf{38.9} & 91.5 & 88.7 & 87.0/90.2 & 80.9 & \textbf{79.5} \\
                \hline
                \rowcolor{gray!10}
                \multicolumn{10}{c}{\textbf{DBKD}} \\
                \hline
                +SVD &  --- & ---/--- & --- & --- & --- & --- & ---/--- & --- & ---\\
                +MPO &  --- & ---/--- & --- & --- & --- & --- & ---/--- & --- & ---\\
                +OPDF & \textbf{69.1} & \textbf{88.4/83.3} & / & \textbf{27.2} & \textbf{88.8} & \textbf{86.5} & \textbf{86.9/90.2} & \textbf{77.6} & \textbf{77.6} \\
                \hline
                \rowcolor{gray!10}
                \multicolumn{10}{c}{\textbf{AD-KD}} \\
                \hline
                +SVD &  --- & ---/--- & --- & --- & --- & --- & ---/--- & --- & ---\\
                +MPO &  --- & ---/--- & --- & --- & --- & --- & ---/--- & --- & ---\\
                +OPDF & \textbf{71.7} & \textbf{90.3/86.8} & 88.9 & \textbf{54.0} & 90.8 & \textbf{91.1} & \textbf{86.4/89.8} & \textbf{82.1} & \textbf{83.2} \\
                \hline
                \end{tabular}
        }
    \caption{Performance comparsion on GLUE benchmark (in percent). "+SVD" represents the use of SVD as the over-parameterization method. "+OPDF" signify the use of OPDF as the over-parameterization method. We show the performance of the model that performs the best on the validation set on the test set. Numbers marked with * indicate that their original paper or released code did not test this task, and the result here were reproduced according to the published code. "Corr." means the average of Pearson and Spearman correlation. The best result for each task is highlight in bold. }
    \label{tab:ablation_result}
\end{table*}

